Communication, and concurrency with logic-based restriction inside a calculus of structures

It is well known that we can use structural proof theory to refine, or generalize, existing paradigmatic computational primitives, or to discover new ones. Under such a point of view we keep developing a programme whose goal is establishing a correspondence between proof-search of a logical system and computations in a process algebra. We give a purely logical account of a process algebra operation which strictly includes the behavior of restriction on actions we find in Milner CCS. This is possible inside a logical system in the Calculus of Structures of Deep Inference endowed with a self-dual quantifier. Using proof-search of cut-free proofs of such a logical system we show how to solve reachability problems in a process algebra that subsumes a significant fragment of Milner CCS.

==> PPi-soundness-example-00.tex <==
For 
every process $ \pincE$, and $ \pincF  $, with $\pincF $ \simple, 
every \standardderivation\ $\bvtDder $, and 
every \environmentstructure\ $ \strR $,
if
$ \vlderivation{
  \vlde{\bvtDder}{\BVTL}
       {\vlsbr[\mapPincToDi{\pincE};\strR]}{
  \vlhy{\mapPincToDi{\pincF}}}} $
then
$\pincLTSJud{\pincE}{\pincF}
            {\mapDiToPinc{\strR}{\emptyset}}$.

==> PPi-soundness-example-01.tex <==
\vlderivation{
  \vlde{\bvtDder'}{\BVTL}
       {\vlsbr[\mapPincToDi{\pincE};\strR]}{
  \vlin{\bvtatrdrule}{(*)}
       {\strS\vlsbr[\atma;\natma]}{
  \vlde{\bvtDder''}{\BVTL}
       {\strS\vlscn{\vlone}}{
  \vlhy{\mapPincToDi{\pincF}}}}}}

==> PPi-soundness-example-02.tex <==
\toks0={3}
\vlderivation{
  \vldf{\scriptsize
        \begin{array}{c}
        \bvtDder''\!\!\\
        \bvtEder' \!\!
        \end{array}
       }{\BVTL}
       {\vlsbr[\mapPincToDi{\pincG};\strR']}{
  \vlhy{\mapPincToDi{\pincF}}}{\the\toks0}}

==> PPi-soundness-example-03.tex <==
  \vlinf{\pinctran}{}
    {\pincLTSJud{\pincE}
		        {\pincF}
		        {\mapDiToPinc{\strR}{\emptyset}}}
    {\pincLTSJud{\pincE}
  		        {\pincG}
		        {\pincLabL}
    \qquad
    \pincLTSJud{\pincG}
		       {\pincF}
  		       {\mapDiToPinc{\strR'}{\emptyset}}}

==> SBV2-example-reduction-01.tex <==
\begin{gathered}
%  \begin{minipage}{.47\textwidth}
%   $$
%   \vlderivation{
%      \vliq{\eqref{align:unit-seq}}{}
%	  {\vlsbr
%	    [\vlfo{\atma}
%		  {[<\atmbBlu;\pincE>;\pincF]}
%	    ;\natmbBlu]
%	  }{
%      \vlin{\bvtseqdrule}{}
%	  {\vlsbr
%	    [\vlfo{\atma}
%		  {[<\atmbBlu;\pincE>
%		    ;<\vlone;\pincF>]}
%	    ;\natmbBlu]
%	  }{
%      \vliq{\eqref{align:unit-pa}
%           ,\eqref{align:alpha-intro}}{}
%	  {\vlsbr
%	    [\vlfo{\atma}
%		  {<[\atmbBlu;\vlone]
%		    ;[\pincE;\pincF]>}
%	    ;\natmbBlu]
%	  }{
%      \vlin{\bvtrdrule}{}
%	  {\vlsbr
%	    [\vlfo{\atma}
%		  {<\atmbBlu
%		    ;[\pincE;\pincF]>}
%	    ;\vlfo{\atma}{\natmbBlu}]
%	  }{
%      \vliq{\eqref{align:unit-seq}}{}
%	  {\vlfo{\atma}
%	    {\vlsbr
%	    [<\atmbBlu
%		;[\pincE;\pincF]>
%	    ;\natmbBlu]
%	    }
%	  }{
%      \vlin{\bvtseqdrule}{}
%	  {\vlfo{\atma}
%	    {\vlsbr
%	    [<\atmbBlu
%		;[\pincE;\pincF]>
%	    ;<\vlone;\natmbBlu>]
%	    }
%	  }{
%      \vliq{\eqref{align:unit-seq}^2}{}
%	  {\vlfo{\atma}
%	    {\vlsbr
%	    <\vlone
%	      ;[<\atmbBlu;[\pincE;\pincF]>
%	      ;\natmbBlu]>
%	    }
%	  }{
%      \vlin{\bvtseqdrule}{}
%	  {\vlfo{\atma}
%	    {\vlsbr
%	      [<\atmbBlu;[\pincE;\pincF]>
%	      ;<\natmbBlu;\vlone>]
%	    }
%	  }{
%      \vliq{\eqref{align:unit-pa}}{}
%	  {\vlfo{\atma}
%	    {\vlsbr
%             <[\atmbBlu;\natmbBlu]
%	      ;[\pincE;\pincF;\vlone]>
%	    }
%	  }{
%      \vliq{\bvtatrdrule
%           ,\eqref{align:unit-seq}}{}
%	  {\vlfo{\atma}
%	    {\vlsbr
%	    <[\atmbBlu;\natmbBlu]
%	      ;[\pincE;\pincF]>
%	    }
%	  }{
%      \vlhy{\vlfo{\atma}
%	    {\vlsbr[\pincE;\pincF]
%	    }
%      }}}}}}}}}}}
%      }
%   $$
%  \end{minipage}
%  %%%% 2nd column
  \begin{minipage}{.45\textwidth}
    $$
    \vlderivation{
      \vliq{}{}
	  {\vlsbr
	    [\vlfo{\atma}
		  {[<\vloneBlu;\pincE>;\pincF]}
	    ;\vloneBlu]
	  }{
      \vlin{}{}
	  {\vlsbr
	    [\vlfo{\atma}
		  {[<\vloneBlu;\pincE>
		    ;<\vlone;\pincF>]}
	    ;\vloneBlu]
	  }{
      \vliq{}{}
	  {\vlsbr
	    [\vlfo{\atma}
		  {<[\vloneBlu;\vlone]
		    ;[\pincE;\pincF]>}
	    ;\vloneBlu]
	  }{
      \vlin{}{}
	  {\vlsbr
	    [\vlfo{\atma}
		  {<\vloneBlu
		    ;[\pincE;\pincF]>}
	    ;\vlfo{\atma}{\vloneBlu}]
	  }{
      \vliq{}{}
	  {\vlfo{\atma}
	    {\vlsbr
	    [<\vloneBlu
		;[\pincE;\pincF]>
	    ;\vloneBlu]
	    }
	  }{
      \vlin{}{}
	  {\vlfo{\atma}
	    {\vlsbr
	    [<\vloneBlu
		;[\pincE;\pincF]>
	    ;<\vlone;\vloneBlu>]
	    }
	  }{
      \vliq{}{}
	  {\vlfo{\atma}
	    {\vlsbr
	    <\vlone
	      ;[<\vloneBlu;[\pincE;\pincF]>
	      ;\vloneBlu]>
	    }
	  }{
      \vlin{}{}
	  {\vlfo{\atma}
	    {\vlsbr
	      [<\vloneBlu;[\pincE;\pincF]>
	      ;<\vloneBlu;\vlone>]
	    }
	  }{
      \vliq{}{}
	  {\vlfo{\atma}
	    {\vlsbr
             <[\vloneBlu;\vloneBlu]
	      ;[\pincE;\pincF;\vlone]>
	    }
	  }{
      \vliq{}{}
	  {\vlfo{\atma}
	    {\vlsbr
	    <[\vloneBlu;\vloneBlu]
	      ;[\pincE;\pincF]>
	    }
	  }{
      \vlhy{\vlfo{\atma}
	             {\vlsbr[\pincE;\pincF]}}}}}}}}}}}}
      }
    $$
  \end{minipage}
\end{gathered}

==> SBV2-standardization-strong.tex <==
\subsection{Full standardization}
\label{subsection:Full standardization}
\paragraph{\OpNameSeq-number of $ \bvtatidrulein $.}
Let $ \bvtPder $ be
$
\vlderivation{
\vldd{\bvtDder'}{\BVT}
     {\strR}{
\vlin{\bvtatidrule}{(*)}
     {\strS\vlsbr[\atma;\natma]}{
\vlpd{\bvtPder'}{\BVT}
     {\strS\vlscn{\vlone}}}}}
     $.
The \OpNameSeq-number of $ (*) $ counts the number of occurrences of \OpNameSeq inside 
$ \strS\vlhole $ to the left-hand side of the redex $ \vlsbr[\atma;\natma] $ of $ (*) $.
Of course \OpNameSeq-number equals zero whenever we can relabel $ (*) $ as $ \bvtatrdrulein $. It is greater than zero, otherwise.
%%%
\begin{proposition}[\textbf{\textit{Commuting conversions in $ \BVT $}}]
\label{proposition:Big-step commuting conversions in BVT}
Let $ \bvtPder $ be
$
\vlderivation{
\vldd{\bvtDder'}{\BVT}
     {\strR}{
\vlin{\bvtatidrule}{(*)}
     {\strS
      \vlsbr<\strT;\strS'[\atma;\natma]>}{
\vlpd{\bvtPder'}{\BVT}
     {\strS
      \vlsbr<\strT;\strS'\,\vlscn{\vlone}>}}}}
     $
with $ (*) $ an instance of $ \bvtatidrulein $ we cannot label $ \bvtatrdrulein $.
There is
$\vlupsmash{
\vlderivation{
\vldd{\bvtDder''}{\BVT}
     {\strR}{
\vlin{\bvtatidrule}{(**)}
     {\strS''\vlsbr[\atma;\natma]}{
\vlpd{\bvtPder''}{\BVT}
     {\strS''\,\vlscn{\vlone}}}}}
}$ without $ (*) $, and such that the \OpNameSeq-number of $ (**) $ is strictly smaller than the \OpNameSeq-number of $ (*) $ in $ \bvtPder $.
\end{proposition}
\begin{proof}
Corollary of Splitting (Point~\ref{enum:Splitting-seq} Theorem~\ref{theorem:Splitting-ALT} in \cite{Roversi:unpub2012-I}), which, we recall, proves that the up-fragment of $ \SBVT $ is admissible for $ \BVT $.
(Details in Appendix~\ref{section:Proof of proposition:Big-step commuting conversions in BVT}.)
\end{proof}
%%%%%%%%%
\paragraph{The fragment $\BVTL$.}
We define $\BVTL$ as the set of rules $ (\BVT\setminus\Set{\bvtatidrulein})\cup \Set{\bvtatrdrulein}$.
So, $ \BVTL $ contains \standardderivation s only, by definition.
Comparing $ \BVTL $ with 
$ \Set{\bvtatrdrulein,\bvtatidrulein,\bvtseqdrulein,\bvtrdrulein} $ in the previous subsection, and whose derivations we know how to make standard, we see we can use both $ \bvtswirulein  $, and $ \bvtatrdrulein $, but not $ \bvtatidrulein $.
%%%%%%%
\begin{theorem}[\textbf{\textit{Completeness of $ \BVTL $ \wrt $ \BVT $}}]
\label{theorem:Partial completeness of BVTL wrt BVT}
For every proof 
$ \bvtInfer{\bvtPder}
           {\ \bvtJudGen{\BVT}
                        {} \strR} $, there exists a \standard proof
$ \bvtInfer{\bvtEder }
           {\ \bvtJudGen{\BVTL}
                        {} \strR} $.
\end{theorem}
%%%%%%%%%
\begin{proof}
By induction on the sum $ s $ of \OpNameSeq-numbers of those $\bvtatidrulein$ in $ \bvtPder$ which cannot be labeled as $\bvtatrdrulein$. Of course, if $s=0$ then $ \bvtPder $ is already in $ \BVTL $, because it only contains instances of $\bvtatrdrulein$, if any. If $ s>0 $, then we stepwise decrease $s$ by iteratively applying Proposition~\ref{proposition:Big-step commuting conversions in BVT}. 
\end{proof}

==> SBV2-tracing-sequential-interactions-02.tex <==
\vlderivation                        {
  \vliq{\eqref{align:unit-seq}}{}
       {\vlsbr
        [<\atmaRed;\strR>
        ;<\natmbBlu;\strT>
        ;<\natmaRed;\atmbBlu>]}        {
  \vlin{\bvtseqdrule}{}
       {\vlsbr
        [<\atmaRed;\strR>
        ;<\vlone;<\natmbBlu;\strT>>
        ;<\natmaRed;\atmbBlu>]}{
  \vliq{\eqref{align:unit-pa}
       ,\eqref{align:unit-seq}}{}
       {\vlsbr
        [<\atmaRed;\strR>
         ;<[\vlone;\natmaRed]
        ;[<\natmbBlu;\strT>;\atmbBlu]>]}{
  \vlin{\bvtseqdrule}{}
       {\vlsbr
        [<\atmaRed;\strR>
         ;<\natmaRed
        ;[<\natmbBlu;\strT>;<\atmbBlu;\vlone>]>]}{
  \vlin{\bvtseqdrule}{}
       {\vlsbr
        [<\atmaRed;\strR>
         ;<\natmaRed
        ;<[\natmbBlu;\atmbBlu];[\strT;\vlone]>>]}{
  \vlin{\bvtatidrule}{}
       {\vlsbr
        <[\atmaRed;\natmaRed]
         ;[\strR
          ;<[\atmbBlu;\natmbBlu];[\strT;\vlone]>]>}{
  \vlin{\bvtatidrule}{}
       {\vlsbr
        <[\atmaRed;\natmaRed]
         ;[\strR
          ;<\vlone;[\strT;\vlone]>]>}{
  \vliq{\eqref{align:unit-seq}^2
       ,\eqref{align:unit-pa}}{}
       {\vlsbr
        <\vlone
         ;[\strR
          ;<\vlone;[\strT;\vlone]>]>}{
  \vlhy{\vlsbr<\strR;\strT>}}}}}}}}}}
